Modelling System of Systems Interface Contract Behaviour

A key challenge in System of Systems (SoS) engineering is the analysis and maintenance of global properties under SoS evolution, and the integration of new constituent elements. There is a need to model the constituent systems composing a SoS in order to allow the analysis of emergent behaviours at the SoS boundary. The Contract pattern allows the engineer to specify constrained behaviours to which constituent systems are required to conform in order to be a part of the SoS. However, the Contract pattern faces some limitations in terms of its accessibility and suitability for verifying contract compatibility. To address these deficiencies, we propose the enrichment of the Contract pattern, which hitherto has been defined using SysML and the COMPASS Modelling Language (CML), by utilising SysML and Object Constraint Language (OCL). In addition, we examine the potential of interface automata, a notation for improving loose coupling between interfaces of constituent systems defined according to the contract, as a means of enabling the verification of contract compatibility. The approach is demonstrated using a case study in audio/video content streaming.

==> eptcsdata.tex <==
\providecommand{\firstpage}{1}
\providecommand{\publicationstatus}{J. Kofro\v{n}, J. Tumova (Eds.): Formal Engineering approaches\\
to Software Components and Architectures (FESCA'17)\\
EPTCS 245, 2017, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.245.1}{10.4204/EPTCS.245.1}}
\pdfoutput=1

